A Multi-Stream Fusion Approach with One-Class Learning for Audio-Visual Deepfake Detection

This paper addresses the challenge of developing a robust audio-visual deepfake detection model. In practical use cases, new generation algorithms are continually emerging, and these algorithms are not encountered during the development of detection methods. This calls for the generalization ability of the method. Additionally, to ensure the credibility of detection methods, it is beneficial for the model to interpret which cues from the video indicate it is fake. Motivated by these considerations, we then propose a multi-stream fusion approach with one-class learning as a representation-level regularization technique. We study the generalization problem of audio-visual deepfake detection by creating a new benchmark by extending and re-splitting the existing FakeAVCeleb dataset. The benchmark contains four categories of fake videos (Real Audio-Fake Visual, Fake Audio-Fake Visual, Fake Audio-Real Visual, and Unsynchronized videos). The experimental results demonstrate that our approach surpasses the previous models by a large margin. Furthermore, our proposed framework offers interpretability, indicating which modality the model identifies as more likely to be fake. The source code is released at https://github.com/bok-bok/MSOC.

==> Figures/oc_figure.tex <==

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/oc_figure.png}
    \caption{Comparison of original softmax and OC-softmax on the binary classification}
    \label{fig:enter-label}
\end{figure}

==> Figures/tsne_modal.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/no_audio.png}
        \caption{Non-OC audio}
        \label{fig:no_audio}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/both_audio.png}
        \caption{OC audio}
        \label{fig:both_audio}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/no_visual.png}
        \caption{Non-OC visual}
        \label{fig:no_visual}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/both_visual.png}
        \caption{OC visual}
        \label{fig:both_visual}
    \end{subfigure}
    \caption{The T-SNE visualization of audio and visual representation computed with models trained with and without OC-softmax.  }
    \label{fig:tsne_each}
\end{figure}


==> Tables/interpret.tex <==


\begin{table}[h]
    \centering
    \caption{Comparison of models trained with and without OC softmax using different feature extractors. The table displays the average \% accuracy and standard deviation of three runs}
    \resizebox{0.5\textwidth}{!}{\begin{tabular}{l|cccc}
        \hline
        \textbf{Branch} & \textbf{Visual} & \textbf{Both} & \textbf{Audio} & \textbf{Unsynced} \\
        \hline

        Audio & $91.00 \pm 3.19$ & $93.33 \pm 2.01$ & $87.83 \pm 5.10$ & $83.67 \pm 4.19$ \\
        Visual & $65.00 \pm 5.72$ & $81.50 \pm 3.27$ & $87.17 \pm 3.06$ & $87.33 \pm 3.01$ \\
        
    \end{tabular}}
    \label{tab:interpret}
\end{table}





==> Tables/loss.tex <==

\begin{table}[h!]
    \centering
    \caption{Summary of Loss Functions}
    \resizebox{0.5\textwidth}{!}{\begin{tabular}{c|ccc}
        \hline
        \textbf{Loss} & \textbf{Features} & \textbf{Label} & \textbf{Center} \\
        \hline
        \(\mathcal{L}_{AOC}^{audio}\) & Audio & Audio & Bonafide audio embeddings of the audio branch \\
        \hline
        \(\mathcal{L}_{VOC}^{visual}\) & Visual & Visual & Bonafide visual embeddings of the visual branch \\
        \hline
        \(\mathcal{L}_{AOC}^{av}\) & Audio & Audio & Bonafide audio embeddings of the audio-visual branch \\
        \hline
        \(\mathcal{L}_{VOC}^{av}\) & Visual & Visual & Bonafide visual embeddings of the audio-visual branch \\
        \hline
    \end{tabular}}
\end{table}
